Characterizing quantum gases in time-controlled disorder realizations using cross-correlations of density distributions

The role of disorder on physical systems has been widely studied in the macroscopic and microscopic world. While static disorder is well understood in many cases, the impact of time-dependent disorder on quantum gases is still poorly investigated. In our experimental setup, we introduce and characterize a method capable of producing time-controlled optical-speckle disorder. Experimentally, coherent light illuminates a combination of a static and a rotating diffuser, thereby collecting a spatially varying phase due to the diffusers' structure and a temporally variable phase due to the relative rotation. Controlling the rotation of the diffuser allows changing the speckle realization or, for future work, the characteristic time scale of the change of the speckle pattern, i.e. the correlation time, matching typical time scales of the quantum gases investigated. We characterize the speckle pattern ex-situ by measuring its intensity distribution cross-correlating different intensity patterns. In-situ, we observe its impact on a molecular Bose-Einstein condensate (BEC) and cross-correlate the density distributions of BECs probed in different speckle realizations. As one diffuser rotates relative to the other around the common optical axis, we trace the optical speckle's intensity cross-correlations and the quantum gas' density cross-correlations. Our results show comparable outcomes for both measurement methods. The setup allows us to tune the disorder potential adapted to the characteristics of the quantum gas. These studies pave the way for investigating nonequilibrium physics in interacting quantum gases using controlled dynamical-disorder potentials.

==> iopart-num.bst.tex <==
% iopart-num.bst -- BibTeX style for IOP journals (Harvard-like numeric style)
% M. A. Caprio
%
% DESCRIPTION
%
%   Further documenation may be found in iopart-num.pdf.
%
%   Available from CTAN as /biblio/bibtex/contrib/iopart-num.
%
% COPYRIGHT/LICENSE
%
%   Copyright 2009 M. A. Caprio
%
%   This work may be distributed and/or modified under the
%   conditions of the LaTeX Project Public License, either 
%   version 1.3 of this license or (at your option) any later 
%   version.  The latest version of this license is in
%     http://www.latex-project.org/lppl.txt
%   and version 1.3 or later is part of all distributions of 
%   LaTeX version 2005/12/01 or later.
%
%   This work has the LPPL maintenance status "maintained".
% 
%   The Current Maintainer of this work is the author.
%
%   The contents of this work are listed in the README file.
%
% HISTORY
% 
% Version 1.0 (2005/07/11)
%   Created using custom-bib (merlin.mbs), with following manual modifications:
%   -- remove trailing period from predefined volume, page, etc., abbreviations
%   -- provide command \newblock to fix incompatibility between natbib
%      and iopart (as of iopart version 1996/06/10) 
%   -- move edition after booktitle
%   -- add version identifier to generated output
%   -- for incollection and inproceedings, move volume from after publisher to before
%   -- for any series with number, number after series
% Version 2.0 (2006/12/21)
%   -- define section field for proper formatting of lettered journal sections 
%      (suggested by Chris Latham)
%   -- suppress printing of number for article, but provide issue field
%      for periodicals with issue-based page numbering (suggested by Chris Latham)
%   -- patch remove.dots to not strip "\." control sequence (bug reported by Kevin Bube)
%   -- define epilog field (undocumented)
%   -- delete predefined computer science journal names
%   -- bring book volume+number or series+number formatting into IOP form
%   -- for book, inbook, and proceedings with editors but no author, fix formating of editors
%   -- for incollection and inproceedings, put editors in correct location
%   -- for journal: use same page formatting even if volume missing
% Version 2.1 (2009/01/22)
%   -- for incollection and inproceedings: support title of chapter (not appropriate 
%      to inbook)
%   -- for book, proceedings, etc.: support volumetitle for multivolume book
%
% LIMITATIONS
%
% Still not in IOP form: 
%   -- for incollection and inproceedings, editors initials should preceed rather 
%      than follow last name
% Other:
%   -- hyphenated first names lose hyphen

%% This is file `iopart-num.bst',
%% generated with the docstrip utility.
%%
%% The original source files were:
%%
%% merlin.mbs  (with options: `seq-no,nm-rv,dt-beg,yr-blk,xmth,yrp-x,jtit-x,vol-bf,volp-blk,num-xser,jnm-x,add-pub,pub-par,pre-pub,isbn,issn,blk-com,com-blank,fin-bare,pp,ed,abr,ednx,mth-bare,ord,jabr,and-xcom,etal-it,revdata,eprint,url,url-blk')
%% ----------------------------------------
%% *** Institute of Physics (IOP) journals; Harvard-like numeric style ***
%% 
%% Copyright 1994-2002 Patrick W Daly
% ===============================================================
% IMPORTANT NOTICE:
% This bibliographic style (bst) file has been generated from one or
% more master bibliographic style (mbs) files, listed above.
%
% This generated file can be redistributed and/or modified under the terms
% of the LaTeX Project Public License Distributed from CTAN
% archives in directory macros/latex/base/lppl.txt; either
% version 1 of the License, or any later version.
% ===============================================================
% Name and version information of the main mbs file:
% \ProvidesFile{merlin.mbs}[2002/10/21 4.05 (PWD, AO, DPC)]
%   For use with BibTeX version 0.99a or later
%-------------------------------------------------------------------
% This bibliography style file is intended for texts in ENGLISH
% This is a numerical citation style, and as such is standard LaTeX.
% It requires no extra package to interface to the main text.
% The form of the \bibitem entries is
%   \bibitem{key}...
% Usage of \cite is as follows:
%   \cite{key} ==>>          [#]
%   \cite[chap. 2]{key} ==>> [#, chap. 2]
% where # is a number determined by the ordering in the reference list.
% The order in the reference list is that by which the works were originally
%   cited in the text, or that in the database.
%---------------------------------------------------------------------

ENTRY
{ address
	archive
	author
	booktitle
	chapter
	collaboration
	edition
	editor
	eid
	eprint
	howpublished
	institution
	isbn
	issn
	journal
	key
	month
	note
	number
	numpages
	organization
	pages
	publisher
	school
	series
	title
	type
	url
	volume
	year
	%mc
	issue
	section
	epilog
	volumetitle
	transjournal
	transsection
	transvolume
	transnumber
	transissue
	transpages
	transyear
}
{}
{ label }

FUNCTION {not}
{   { #0 }
	{ #1 }
	if$
}
FUNCTION {and}
{   'skip$
	{ pop$ #0 }
	if$
}
FUNCTION {or}
{   { pop$ #1 }
	'skip$
	if$
}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% mc utilities
%   require merlin.mbs logical operators and field.or.null
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

% hang -- {hang} suspends execution, for debugging purposes
%   Note that not all pending output may have been flushed.
FUNCTION {hang}
{
	{#1} {skip$} while$
}

% string.length -- {s string.length} returns the true character length of s
%   In contrast, text.length$ gives special treatment to LaTeX
%   accents ("special characters") and braces.
%   Example:   "" string.length     -> 0
%   Example:   "hello" string.length    -> 5

STRINGS {string.length.s }
INTEGERS {string.length.i }
FUNCTION {string.length}
{
	'string.length.s :=
	#0 'string.length.i :=
	{
		string.length.s #1 #1 substring$ "" = not
	}
	{ 
		string.length.i #1 + 'string.length.i := 
		string.length.s #2 global.max$ substring$ 'string.length.s :=
	}
	while$
	string.length.i
}

% shared working variables for stripping functions
STRINGS { strip.s strip.t }
INTEGERS { strip.i }

% strip.leading -- {s t strip.leading} strips t from s if it appears
%   as an initial substring 
%   Example:   "abcdef" "abc" strip.leading   -> "def"
%   Example:   "abcdef" "xyz" strip.leading   -> "abcdef"

FUNCTION{strip.leading}
{
	'strip.t :=
	'strip.s :=
	strip.t string.length 'strip.i :=
	strip.s #1 strip.i substring$ strip.t =
	{ strip.s strip.i #1 + global.max$ substring$ }
	{ strip.s }
	if$
}

% strip.trailing -- {s t strip.trailing} strips t from s if it appears
%   as a terminal substring 
%   Example:   "abcdef" "def" strip.trailing  -> "abc"
%   Example:   "abcdef" "xyz" strip.trailing  -> "abcdef"
FUNCTION{strip.trailing}
{
	'strip.t :=
	'strip.s :=
	strip.t string.length 'strip.i :=
	strip.s #-1 strip.i substring$ strip.t =
	{ strip.s #-1 strip.i - global.max$ substring$ }
	{ strip.s }
	if$
}

% trim -- {s trim} strips any trailing whitespace from s
%   Example:   "abcdef  " trim  -> "abcdef"
STRINGS {trim.s trim.t}
FUNCTION{trim}
{
	'trim.s :=
	{
		trim.s #-1 #1 substring$ 'trim.t :=
		trim.t empty$ trim.t string.length #0 > and
	}
	{ trim.s #-2 global.max$ substring$ 'trim.s := }
	while$
	trim.s
}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


INTEGERS { output.state before.all mid.sentence after.sentence after.block }
FUNCTION {init.state.consts}
{ #0 'before.all :=
	#1 'mid.sentence :=
	#2 'after.sentence :=
	#3 'after.block :=
}
STRINGS { s t}

FUNCTION {output.nonnull}
{ 's :=
	output.state mid.sentence =
	{ " " * write$ }
	{ output.state after.block =
		{ add.period$ write$
			newline$
			"\newblock " write$
		}
		{ output.state before.all =
			'write$
			{ add.period$ " " * write$ }
			if$
		}
		if$
		mid.sentence 'output.state :=
	}
	if$
	s
}
FUNCTION {output}
{ duplicate$ empty$
	'pop$
	'output.nonnull
	if$
}
FUNCTION {output.check}
{ 't :=
	duplicate$ empty$
	{ pop$ "empty " t * " in " * cite$ * warning$ }
	'output.nonnull
	if$
}

%mc
FUNCTION {format.epilog}
{ epilog duplicate$ empty$
	{ pop$ }
	{ * }
	if$
}
%mc end


FUNCTION {fin.entry}
{   
	%mc
	format.epilog 
	%mc end
	duplicate$ empty$
	'pop$
	'write$
	if$
	newline$
}

FUNCTION {new.block}
{ output.state before.all =
	'skip$
	{ after.block 'output.state := }
	if$
}
FUNCTION {new.sentence}
{ output.state after.block =
	'skip$
	{ output.state before.all =
		'skip$
		{ after.sentence 'output.state := }
		if$
	}
	if$
}
FUNCTION {add.blank}
{  " " * before.all 'output.state :=
}

FUNCTION {date.block}
{
	add.blank
}

STRINGS {z}
FUNCTION {remove.dots}
{ 'z :=
	""
	{ z empty$ not }
	{
		%mc patch to preserve the control sequence \. if it appears in a name
		z #1 #2 substring$ "\." = 
		{ 
			% process "\." sequence
			z #3 global.max$ substring$ 'z :=
			"\." * 
		}
		{    
			% process regular character
			z #1 #1 substring$
			z #2 global.max$ substring$ 'z :=
			duplicate$ "." = 'pop$
			{ * }
			if$
		}
		if$
		%mc
	}
	while$
}
FUNCTION {new.block.checka}
{ empty$
	'skip$
	'new.block
	if$
}
FUNCTION {new.block.checkb}
{ empty$
	swap$ empty$
	and
	'skip$
	'new.block
	if$
}
FUNCTION {new.sentence.checka}
{ empty$
	'skip$
	'new.sentence
	if$
}
FUNCTION {new.sentence.checkb}
{ empty$
	swap$ empty$
	and
	'skip$
	'new.sentence
	if$
}
FUNCTION {field.or.null}
{ duplicate$ empty$
	{ pop$ "" }
	'skip$
	if$
}
FUNCTION {emphasize}
{ duplicate$ empty$
	{ pop$ "" }
	{ "{\em " swap$ * "\/}" * }
	if$
}
FUNCTION {bolden}
{ duplicate$ empty$
	{ pop$ "" }
	{ "{\bf " swap$ * "}" * }
	if$
}
FUNCTION {tie.or.space.prefix}
{ duplicate$ text.length$ #3 <
	{ "~" }
	{ " " }
	if$
	swap$
}

FUNCTION {capitalize}
{ "u" change.case$ "t" change.case$ }

FUNCTION {space.word}
{ " " swap$ * " " * }
% Here are the language-specific definitions for explicit words.
% Each function has a name bbl.xxx where xxx is the English word.
% The language selected here is ENGLISH
FUNCTION {bbl.and}
{ "and"}

FUNCTION {bbl.etal}
{ "et~al." }

FUNCTION {bbl.editors}
{ "eds" }

FUNCTION {bbl.editor}
{ "ed" }

FUNCTION {bbl.edby}
{ "edited by" }

FUNCTION {bbl.edition}
{ "ed" }

FUNCTION {bbl.volume}
{ "vol" }

FUNCTION {bbl.of}
{ "of" }

FUNCTION {bbl.number}
{ "no" }

FUNCTION {bbl.nr}
{ "no" }

FUNCTION {bbl.in}
{ "in" }

FUNCTION {bbl.pages}
{ "pp" }

FUNCTION {bbl.page}
{ "p" }

FUNCTION {bbl.eidpp}
{ "pages" }

FUNCTION {bbl.chapter}
{ "chap" }

FUNCTION {bbl.techrep}
{ "Tech. Rep." }

FUNCTION {bbl.mthesis}
{ "Master's thesis" }

FUNCTION {bbl.phdthesis}
{ "Ph.D. thesis" }

FUNCTION {bbl.first}
{ "1st" }

FUNCTION {bbl.second}
{ "2nd" }

FUNCTION {bbl.third}
{ "3rd" }

FUNCTION {bbl.fourth}
{ "4th" }

FUNCTION {bbl.fifth}
{ "5th" }

FUNCTION {bbl.st}
{ "st" }

FUNCTION {bbl.nd}
{ "nd" }

FUNCTION {bbl.rd}
{ "rd" }

FUNCTION {bbl.th}
{ "th" }

MACRO {jan} {"Jan."}

MACRO {feb} {"Feb."}

MACRO {mar} {"Mar."}

MACRO {apr} {"Apr."}

MACRO {may} {"May"}

MACRO {jun} {"Jun."}

MACRO {jul} {"Jul."}

MACRO {aug} {"Aug."}

MACRO {sep} {"Sep."}

MACRO {oct} {"Oct."}

MACRO {nov} {"Nov."}

MACRO {dec} {"Dec."}

FUNCTION {eng.ord}
{ duplicate$ "1" swap$ *
	#-2 #1 substring$ "1" =
	{ bbl.th * }
	{ duplicate$ #-1 #1 substring$
		duplicate$ "1" =
		{ pop$ bbl.st * }
		{ duplicate$ "2" =
			{ pop$ bbl.nd * }
			{ "3" =
				{ bbl.rd * }
				{ bbl.th * }
				if$
			}
			if$
		}
		if$
	}
	if$
}

FUNCTION {bibinfo.check}
{ swap$
	duplicate$ missing$
	{
		pop$ pop$
		""
	}
	{ duplicate$ empty$
		{
			swap$ pop$
		}
		{ swap$
			pop$
		}
		if$
	}
	if$
}
FUNCTION {bibinfo.warn}
{ swap$
	duplicate$ missing$
	{
		swap$ "missing " swap$ * " in " * cite$ * warning$ pop$
		""
	}
	{ duplicate$ empty$
		{
			swap$ "empty " swap$ * " in " * cite$ * warning$
		}
		{ swap$
			pop$
		}
		if$
	}
	if$
}
%% FUNCTION {format.eprint}
%% { eprint duplicate$ empty$
	%%     'skip$
	%%     { "\eprint"
		%%       archive empty$
		%%         'skip$
		%%         { "[" * archive * "]" * }
		%%       if$
		%%       "{" * swap$ * "}" *
		%%     }
	%%   if$
	%% }
FUNCTION {format.eprint}
{ eprint duplicate$ empty$
	'skip$
	{ 
		"(\textit{Preprint} " 
		swap$
		"\eprint"
		archive empty$
		'skip$
		{ "[" * archive * "]" * }
		if$
		"{" * swap$ * "}" *
		*
		")"
		*
	}
	if$
}

FUNCTION {format.url}
{ url empty$
	{ "" }
	{ "\urlprefix\url{" url * "}" * }
	if$
}

STRINGS  { bibinfo}
INTEGERS { nameptr namesleft numnames }

FUNCTION {format.names}
{ 'bibinfo :=
	duplicate$ empty$ 'skip$ {
		's :=
		"" 't :=
		#1 'nameptr :=
		s num.names$ 'numnames :=
		numnames 'namesleft :=
		{ namesleft #0 > }
		{ s nameptr
			"{vv~}{ll}{ jj}{ f{~}}"
			format.name$
			remove.dots
			bibinfo bibinfo.check
			't :=
			nameptr #1 >
			{
				namesleft #1 >
				{ ", " * t * }
				{
					s nameptr "{ll}" format.name$ duplicate$ "others" =
					{ 't := }
					{ pop$ }
					if$
					t "others" =
					{
						" " * bbl.etal emphasize *
					}
					{
						bbl.and
						space.word * t *
					}
					if$
				}
				if$
			}
			't
			if$
			nameptr #1 + 'nameptr :=
			namesleft #1 - 'namesleft :=
		}
		while$
	} if$
}
FUNCTION {format.names.ed}
{
	'bibinfo :=
	duplicate$ empty$ 'skip$ {
		's :=
		"" 't :=
		#1 'nameptr :=
		s num.names$ 'numnames :=
		numnames 'namesleft :=
		{ namesleft #0 > }
		{ s nameptr
			"{f{~}~}{vv~}{ll}{ jj}"
			format.name$
			remove.dots
			bibinfo bibinfo.check
			't :=
			nameptr #1 >
			{
				namesleft #1 >
				{ ", " * t * }
				{
					s nameptr "{ll}" format.name$ duplicate$ "others" =
					{ 't := }
					{ pop$ }
					if$
					t "others" =
					{
						
						" " * bbl.etal emphasize *
					}
					{
						bbl.and
						space.word * t *
					}
					if$
				}
				if$
			}
			't
			if$
			nameptr #1 + 'nameptr :=
			namesleft #1 - 'namesleft :=
		}
		while$
	} if$
}
FUNCTION {format.authors}
{ author "author" format.names
	duplicate$ empty$ 'skip$
	{ collaboration "collaboration" bibinfo.check
		duplicate$ empty$ 'skip$
		{ " (" swap$ * ")" * }
		if$
		*
	}
	if$
}
FUNCTION {get.bbl.editor}
{ editor num.names$ #1 > 'bbl.editors 'bbl.editor if$ }

FUNCTION {format.editors}
{ editor "editor" format.names duplicate$ empty$ 'skip$
	{
		%%      "," *
		%%      " " *
		%%      get.bbl.editor
		%%      *
		%mc
		" " *
		"(" *
		get.bbl.editor
		*
		")" *
		%mc end
	}
	if$
}
%mc
FUNCTION {format.editors.inline}
{ editor "editor" format.names duplicate$ empty$ 'skip$
	{
		bbl.editor " " *
		swap$
		*
	}
	if$
}
%mc end

FUNCTION {format.isbn}
{ isbn "isbn" bibinfo.check
	duplicate$ empty$ 'skip$
	{
		"ISBN " swap$ *
	}
	if$
}

FUNCTION {format.issn}
{ issn "issn" bibinfo.check
	duplicate$ empty$ 'skip$
	{
		"ISSN " swap$ *
	}
	if$
}

FUNCTION {format.note}
{
	note empty$
	{ "" }
	{ note #1 #1 substring$
		duplicate$ "{" =
			'skip$
			{ output.state mid.sentence =
				{ "l" }
				{ "u" }
				if$
				change.case$
			}
			if$
			note #2 global.max$ substring$ * "note" bibinfo.check
		}
		if$
	}
	
	FUNCTION {format.title}
	{ title
		duplicate$ empty$ 'skip$
		{ "t" change.case$ }
		if$
		"title" bibinfo.check
	}
	FUNCTION {output.bibitem}
	{ newline$
		"\bibitem{" write$
			cite$ write$
			"}" write$
		newline$
		""
		before.all 'output.state :=
	}
	
	FUNCTION {n.dashify}
	{
		't :=
		""
		{ t empty$ not }
		{ t #1 #1 substring$ "-" =
			{ t #1 #2 substring$ "--" = not
				{ "--" *
					t #2 global.max$ substring$ 't :=
				}
				{   { t #1 #1 substring$ "-" = }
					{ "-" *
						t #2 global.max$ substring$ 't :=
					}
					while$
				}
				if$
			}
			{ t #1 #1 substring$ *
				t #2 global.max$ substring$ 't :=
			}
			if$
		}
		while$
	}
	
	FUNCTION {word.in}
	{ bbl.in
		" " * }
	
	FUNCTION {format.date}
	{
		""
		duplicate$ empty$
		year  "year"  bibinfo.check duplicate$ empty$
		{ swap$ 'skip$
			{ "there's a month but no year in " cite$ * warning$ }
			if$
			*
		}
		{ swap$ 'skip$
			{
				swap$
				" " * swap$
			}
			if$
			*
			remove.dots
		}
		if$
		duplicate$ empty$
		'skip$
		{
			before.all 'output.state :=
			" " swap$ *
		}
		if$
	}
	FUNCTION {format.btitle}
	{ title "title" bibinfo.check
		duplicate$ empty$ 'skip$
		{
			emphasize
		}
		if$
	}
	FUNCTION {either.or.check}
	{ empty$
		'pop$
		{ "can't use both " swap$ * " fields in " * cite$ * warning$ }
		if$
	}
	FUNCTION {format.bvolume}
	{ volume empty$
		% no volume: return blank
		{ "" }
		%%    { bbl.volume volume tie.or.space.prefix
			%%      "volume" bibinfo.check * *
			%%      series "series" bibinfo.check
			%%      duplicate$ empty$ 'pop$
			%%        { swap$ bbl.of space.word * swap$
				%%         emphasize * }
			%%      if$
			%%      "volume and number" number either.or.check
			%%    }
		%mc
		{
			series "series" bibinfo.check
			empty$ 
			% no series: must be multivolume book
			{
				bbl.volume volume tie.or.space.prefix "volume" bibinfo.check * *
				volumetitle empty$
				'skip$
				% volumetitle: book volume has title
				{ " " volumetitle "volumetitle" bibinfo.check emphasize * * }
				if$
			}
			% series: format as volume in series
			{ 
				"(" 
				series "series" bibinfo.check emphasize *
				" " * bbl.volume * 
				volume tie.or.space.prefix "volume" bibinfo.check * 
				")" * *
			}
			if$
			"volume and number" number either.or.check
		}
		%mc end
		if$
	}
	FUNCTION {format.number.series}
	{ volume empty$
		{ number empty$
			{ series field.or.null }
			{ series empty$
				{ number "number" bibinfo.check }
				{ 
					%% output.state mid.sentence =
					%%   { bbl.number }
					%%   { bbl.number capitalize }
					%% if$
					%% number tie.or.space.prefix "number" bibinfo.check * *
					%% bbl.in space.word *
					%% series "series" bibinfo.check *
					%% " " * bbl.number * 
					%% number tie.or.space.prefix "number" bibinfo.check * *
					%mc
					"(" 
					series "series" bibinfo.check emphasize *
					" " * bbl.number * 
					number tie.or.space.prefix "number" bibinfo.check * 
					")" *
					*
					%mc end
				}
				if$
			}
			if$
		}
		{ "" }
		if$
	}
	
	
	FUNCTION {is.num}
	{ chr.to.int$
		duplicate$ "0" chr.to.int$ < not
		swap$ "9" chr.to.int$ > not and
	}
	
	FUNCTION {extract.num}
	{ duplicate$ 't :=
		"" 's :=
		{ t empty$ not }
		{ t #1 #1 substring$
			t #2 global.max$ substring$ 't :=
			duplicate$ is.num
			{ s swap$ * 's := }
			{ pop$ "" 't := }
			if$
		}
		while$
		s empty$
		'skip$
		{ pop$ s }
		if$
	}
	
	FUNCTION {convert.edition}
	{ extract.num "l" change.case$ 's :=
		s "first" = s "1" = or
		{ bbl.first 't := }
		{ s "second" = s "2" = or
			{ bbl.second 't := }
			{ s "third" = s "3" = or
				{ bbl.third 't := }
				{ s "fourth" = s "4" = or
					{ bbl.fourth 't := }
					{ s "fifth" = s "5" = or
						{ bbl.fifth 't := }
						{ s #1 #1 substring$ is.num
							{ s eng.ord 't := }
							{ edition 't := }
							if$
						}
						if$
					}
					if$
				}
				if$
			}
			if$
		}
		if$
		t
	}
	
	FUNCTION {format.edition}
	{ edition duplicate$ empty$ 'skip$
		{
			convert.edition
			output.state mid.sentence =
			{ "l" }
			{ "t" }
			if$ change.case$
			"edition" bibinfo.check
			" " * bbl.edition *
		}
		if$
	}
	INTEGERS { multiresult }
	FUNCTION {multi.page.check}
	{ 't :=
		#0 'multiresult :=
		{ multiresult not
			t empty$ not
			and
		}
		{ t #1 #1 substring$
			duplicate$ "-" =
			swap$ duplicate$ "," =
			swap$ "+" =
			or or
			{ #1 'multiresult := }
			{ t #2 global.max$ substring$ 't := }
			if$
		}
		while$
		multiresult
	}
	FUNCTION {format.pages}
	{ pages duplicate$ empty$ 'skip$
		{ duplicate$ multi.page.check
			{
				bbl.pages swap$
				n.dashify
			}
			{
				bbl.page swap$
			}
			if$
			tie.or.space.prefix
			"pages" bibinfo.check
			* *
		}
		if$
	}
	FUNCTION {format.journal.pages}
	{ pages duplicate$ empty$ 'pop$
		%mc     { swap$ duplicate$ empty$
			%mc         { pop$ pop$ format.pages }
			%mc         {
				%mc           " " *
				%mc           swap$
				%mc           n.dashify
				%mc           "pages" bibinfo.check
				%mc           *
				%mc         }
			%mc       if$
			%mc     }
		{ swap$
			" " *
			swap$
			n.dashify
			"pages" bibinfo.check
			*
		}
		if$
	}
	FUNCTION {format.journal.eid}
	{ eid "eid" bibinfo.check
		duplicate$ empty$ 'skip$
		{ swap$ duplicate$ empty$ 'skip$
			{
				" " *
			}
			if$
			swap$
			numpages empty$ 'skip$
			{ bbl.eidpp numpages tie.or.space.prefix
				"numpages" bibinfo.check * *
				" (" swap$ * ")" * *
			}
			if$
		}
		if$ *
	}
	FUNCTION {format.vol.num.pages}
	{ volume field.or.null
		%mc section handling
		section field.or.null strip.leading
		section field.or.null strip.trailing trim
		%mc end
		duplicate$ empty$ 'skip$
		{
			"volume" bibinfo.check
		}
		if$
		bolden
		%mc  number "number" bibinfo.check duplicate$ empty$ 'skip$
		issue "issue" bibinfo.check duplicate$ empty$ 'skip$
		{
			swap$ duplicate$ empty$
			%mc        { "there's a number but no volume in " cite$ * warning$ }
			{ "there's an issue but no volume in " cite$ * warning$ }
			'skip$
			if$
			swap$
			"(" swap$ * ")" *
		}
		if$ *
		eid empty$
		{ format.journal.pages }
		{ format.journal.eid }
		if$
	}
	
	FUNCTION {format.chapter.pages}
	{ chapter empty$
		'format.pages
		{ type empty$
			{ bbl.chapter }
			{ type "l" change.case$
				"type" bibinfo.check
			}
			if$
			chapter tie.or.space.prefix
			"chapter" bibinfo.check
			* *
			pages empty$
			'skip$
			{ ", " * format.pages * }
			if$
		}
		if$
	}
	
	FUNCTION {format.booktitle}
	{
		booktitle "booktitle" bibinfo.check
		emphasize
	}
	%% FUNCTION {format.in.ed.booktitle}
	%% { format.booktitle duplicate$ empty$ 'skip$
		%%     {
			%%       editor "editor" format.names.ed duplicate$ empty$ 'pop$
			%%         {
				%%           "," *
				%%           " " *
				%%           get.bbl.editor
				%%           ", " *
				%%           * swap$
				%%           * }
			%%       if$
			%%       word.in swap$ *
			%%     }
		%%   if$
		%% }
	FUNCTION {empty.misc.check}
	{ author empty$ title empty$ howpublished empty$
		month empty$ year empty$ note empty$
		and and and and and
		{ "all relevant fields are empty in " cite$ * warning$ }
		'skip$
		if$
	}
	FUNCTION {format.thesis.type}
	{ type duplicate$ empty$
		'pop$
		{ swap$ pop$
			"t" change.case$ "type" bibinfo.check
		}
		if$
	}
	FUNCTION {format.tr.number}
	{ number "number" bibinfo.check
		type duplicate$ empty$
		{ pop$ bbl.techrep }
		'skip$
		if$
		"type" bibinfo.check
		swap$ duplicate$ empty$
		{ pop$ "t" change.case$ }
		{ tie.or.space.prefix * * }
		if$
	}
	FUNCTION {format.article.crossref}
	{
		key duplicate$ empty$
		{ pop$
			journal duplicate$ empty$
			{ "need key or journal for " cite$ * " to crossref " * crossref * warning$ }
			{ "journal" bibinfo.check emphasize word.in swap$ * }
			if$
		}
		{ word.in swap$ * " " *}
		if$
		" \cite{" * crossref * "}" *
	}
	FUNCTION {format.crossref.editor}
	{ editor #1 "{vv~}{ll}" format.name$
		"editor" bibinfo.check
		editor num.names$ duplicate$
		#2 >
		{ pop$
			"editor" bibinfo.check
			" " * bbl.etal
			emphasize
			*
		}
		{ #2 <
			'skip$
			{ editor #2 "{ff }{vv }{ll}{ jj}" format.name$ "others" =
				{
					"editor" bibinfo.check
					" " * bbl.etal
					emphasize
					*
				}
				{
					bbl.and space.word
					* editor #2 "{vv~}{ll}" format.name$
					"editor" bibinfo.check
					*
				}
				if$
			}
			if$
		}
		if$
	}
	
	FUNCTION {format.book.crossref}
	{ volume duplicate$ empty$
		{ "empty volume in " cite$ * "'s crossref of " * crossref * warning$
			pop$ word.in
		}
		{ bbl.volume
			swap$ tie.or.space.prefix "volume" bibinfo.check * * bbl.of space.word *
		}
		if$
		editor empty$
		editor field.or.null author field.or.null =
		or
		{ key empty$
			{ series empty$
				{ "need editor, key, or series for " cite$ * " to crossref " *
					crossref * warning$
					"" *
				}
				{ series emphasize * }
				if$
			}
			{ key * }
			if$
		}
		{ format.crossref.editor * }
		if$
		" \cite{" * crossref * "}" *
	}
	FUNCTION {format.incoll.inproc.crossref}
	{
		editor empty$
		editor field.or.null author field.or.null =
		or
		{ key empty$
			{ format.booktitle duplicate$ empty$
				{ "need editor, key, or booktitle for " cite$ * " to crossref " *
					crossref * warning$
				}
				{ word.in swap$ * }
				if$
			}
			{ word.in key * " " *}
			if$
		}
		{ word.in format.crossref.editor * " " *}
		if$
		" \cite{" * crossref * "}" *
	}
	FUNCTION {format.org.or.pub}
	{ 't :=
		""
		address empty$ t empty$ and
		'skip$
		{
			add.blank "(" *
			address "address" bibinfo.check *
			t empty$
			'skip$
			{ address empty$
				'skip$
				{ ": " * }
				if$
				t *
			}
			if$
			")" *
		}
		if$
	}
	FUNCTION {format.publisher.address}
	{ publisher "publisher" bibinfo.warn format.org.or.pub
	}
	
	FUNCTION {format.organization.address}
	{ organization "organization" bibinfo.check format.org.or.pub
	}
	
	
	
	FUNCTION {article}
	{ output.bibitem
		format.authors "author" output.check
		format.date "year" output.check
		date.block
		crossref missing$
		{
			%mc add section handling
			%mc       journal
			%mc       "journal" bibinfo.check
			%mc       emphasize
			%mc       "journal" output.check
			%mc       add.blank
			journal
			"journal" bibinfo.check
			section field.or.null strip.trailing trim
			emphasize
			"journal" output.check
			add.blank
			section empty$
			{ skip$ }
			{ section * add.blank}
			if$
			%mc end
			format.vol.num.pages output
		}
		{ format.article.crossref output.nonnull
			format.pages output
		}
		if$
		format.issn output
		format.note output
		format.eprint output
		format.url output
		fin.entry
	}
	FUNCTION {book}
	{ output.bibitem
		author empty$
		{ format.editors "author and editor" output.check
		}
		{ format.authors output.nonnull
			crossref missing$
			{ "author and editor" editor either.or.check }
			'skip$
			if$
		}
		if$
		format.date "year" output.check
		date.block
		format.btitle "title" output.check
		format.edition output
		crossref missing$
		{ format.bvolume output
			format.number.series output
			format.publisher.address output
		}
		{
			format.book.crossref output.nonnull
		}
		if$
		%% format.edition output
		format.isbn output
		format.note output
		format.eprint output
		format.url output
		fin.entry
	}
	FUNCTION {booklet}
	{ output.bibitem
		format.authors output
		format.date output
		date.block
		format.title "title" output.check
		howpublished "howpublished" bibinfo.check output
		address "address" bibinfo.check output
		format.isbn output
		format.note output
		format.eprint output
		format.url output
		fin.entry
	}
	
	FUNCTION {inbook}
	{ output.bibitem
		author empty$
		{ format.editors "author and editor" output.check
		}
		{ format.authors output.nonnull
			crossref missing$
			{ "author and editor" editor either.or.check }
			'skip$
			if$
		}
		if$
		format.date "year" output.check
		date.block
		format.btitle "title" output.check
		crossref missing$
		{
			format.bvolume output
			format.publisher.address output
			%% format.bvolume output
			format.chapter.pages "chapter and pages" output.check
			format.number.series output
		}
		{
			format.chapter.pages "chapter and pages" output.check
			format.book.crossref output.nonnull
		}
		if$
		format.edition output
		crossref missing$
		{ format.isbn output }
		'skip$
		if$
		format.note output
		format.eprint output
		format.url output
		fin.entry
	}
	
	FUNCTION {incollection}
	{ output.bibitem
		format.authors "author" output.check
		format.date "year" output.check
		date.block
		format.title "title" output.check
		crossref missing$
		{ 
			%% format.in.ed.booktitle "booktitle" output.check
			%mc   
			format.booktitle "booktitle" output.check
			format.bvolume output
			format.number.series output
			format.editors.inline output
			%mc end
			format.publisher.address output
			%% format.bvolume output
			%% format.number.series output
			format.chapter.pages output
			format.edition output
			format.isbn output
		}
		{ format.incoll.inproc.crossref output.nonnull
			format.chapter.pages output
		}
		if$
		format.note output
		format.eprint output
		format.url output
		fin.entry
	}
	FUNCTION {inproceedings}
	{ output.bibitem
		format.authors "author" output.check
		format.date "year" output.check
		date.block
		format.title "title" output.check
		crossref missing$
		{ 
			
			%%format.in.ed.booktitle "booktitle" output.check
			%mc   
			format.booktitle "booktitle" output.check
			format.bvolume output
			format.number.series output
			format.editors.inline output
			%mc end
			publisher empty$
			{ format.organization.address output }
			{ organization "organization" bibinfo.check output
				format.publisher.address output
			}
			if$
			%% format.bvolume output
			%% format.number.series output
			format.pages output
			format.isbn output
			format.issn output
		}
		{ format.incoll.inproc.crossref output.nonnull
			format.pages output
		}
		if$
		format.note output
		format.eprint output
		format.url output
		fin.entry
	}
	FUNCTION {conference} { inproceedings }
	FUNCTION {manual}
	{ output.bibitem
		author empty$
		{ organization "organization" bibinfo.check
			duplicate$ empty$ 'pop$
			{ output
				address "address" bibinfo.check output
			}
			if$
		}
		{ format.authors output.nonnull }
		if$
		format.date output
		date.block
		format.btitle "title" output.check
		author empty$
		{ organization empty$
			{
				address "address" bibinfo.check output
			}
			'skip$
			if$
		}
		{
			organization "organization" bibinfo.check output
			address "address" bibinfo.check output
		}
		if$
		format.edition output
		format.note output
		format.eprint output
		format.url output
		fin.entry
	}
	
	FUNCTION {mastersthesis}
	{ output.bibitem
		format.authors "author" output.check
		format.date "year" output.check
		date.block
		format.btitle
		"title" output.check
		bbl.mthesis format.thesis.type output.nonnull
		school "school" bibinfo.warn output
		address "address" bibinfo.check output
		format.note output
		format.eprint output
		format.url output
		fin.entry
	}
	
	FUNCTION {misc}
	{ output.bibitem
		format.authors output
		format.date output
		format.title output
		howpublished "howpublished" bibinfo.check output
		format.note output
		format.eprint output
		format.url output
		fin.entry
		empty.misc.check
	}
	FUNCTION {phdthesis}
	{ output.bibitem
		format.authors "author" output.check
		format.date "year" output.check
		date.block
		format.btitle
		"title" output.check
		bbl.phdthesis format.thesis.type output.nonnull
		school "school" bibinfo.warn output
		address "address" bibinfo.check output
		format.note output
		format.eprint output
		format.url output
		fin.entry
	}
	
	FUNCTION {proceedings}
	{ output.bibitem
		editor empty$
		{ organization "organization" bibinfo.check output
		}
		{ format.editors output.nonnull }
		if$
		format.date "year" output.check
		date.block
		format.btitle "title" output.check
		format.bvolume output
		format.number.series output
		editor empty$
		{ publisher empty$
			'skip$
			{
				format.publisher.address output
			}
			if$
		}
		{ publisher empty$
			{
				format.organization.address output }
			{
				organization "organization" bibinfo.check output
				format.publisher.address output
			}
			if$
		}
		if$
		format.isbn output
		format.issn output
		format.note output
		format.eprint output
		format.url output
		fin.entry
	}
	
	FUNCTION {techreport}
	{ output.bibitem
		format.authors "author" output.check
		format.date "year" output.check
		date.block
		format.title
		"title" output.check
		format.tr.number output.nonnull
		institution "institution" bibinfo.warn output
		address "address" bibinfo.check output
		format.note output
		format.eprint output
		format.url output
		fin.entry
	}
	
	FUNCTION {unpublished}
	{ output.bibitem
		format.authors "author" output.check
		format.date output
		date.block
		format.title "title" output.check
		format.note "note" output.check
		format.eprint output
		format.url output
		fin.entry
	}
	
	FUNCTION {default.type} { misc }
	READ
	STRINGS { longest.label }
	INTEGERS { number.label longest.label.width }
	FUNCTION {initialize.longest.label}
	{ "" 'longest.label :=
		#1 'number.label :=
		#0 'longest.label.width :=
	}
	FUNCTION {longest.label.pass}
	{ number.label int.to.str$ 'label :=
		number.label #1 + 'number.label :=
		label width$ longest.label.width >
		{ label 'longest.label :=
			label width$ 'longest.label.width :=
		}
		'skip$
		if$
	}
	EXECUTE {initialize.longest.label}
	ITERATE {longest.label.pass}
	FUNCTION {begin.bib}
	{ preamble$ empty$
		'skip$
		{ preamble$ write$ newline$ }
		if$
		"\providecommand{\newblock}{}"
		write$ newline$
		"\begin{thebibliography}{"  longest.label  * "}" *
			write$ newline$
			"\expandafter\ifx\csname url\endcsname\relax"
			write$ newline$
			"  \def\url#1{{\tt #1}}\fi"
			write$ newline$
			"\expandafter\ifx\csname urlprefix\endcsname\relax\def\urlprefix{URL }\fi"
			write$ newline$
			"\providecommand{\eprint}[2][]{\url{#2}}"
			write$ newline$
			"% Bibliography created with iopart-num v2.1"
			write$ newline$
			"% /biblio/bibtex/contrib/iopart-num"
			write$ newline$
		}
		EXECUTE {begin.bib}
		EXECUTE {init.state.consts}
		ITERATE {call.type$}
		FUNCTION {end.bib}
		{ newline$
			"\end{thebibliography}" write$ newline$
	}
	EXECUTE {end.bib}
	%% End of customized bst file
	%%
	%% End of file `iopart-num.bst'.
